VALUE: A Multi-Task Benchmark for Video-and-Language Understanding Evaluation

Most existing video-and-language (VidL) research focuses on a single dataset, or multiple datasets of a single task. In reality, a truly useful VidL system is expected to be easily generalizable to diverse tasks, domains, and datasets. To facilitate the evaluation of such systems, we introduce Video-And-Language Understanding Evaluation (VALUE) benchmark, an assemblage of 11 VidL datasets over 3 popular tasks: (i) text-to-video retrieval; (ii) video question answering; and (iii) video captioning. VALUE benchmark aims to cover a broad range of video genres, video lengths, data volumes, and task difficulty levels. Rather than focusing on single-channel videos with visual information only, VALUE promotes models that leverage information from both video frames and their associated subtitles, as well as models that share knowledge across multiple tasks. We evaluate various baseline methods with and without large-scale VidL pre-training, and systematically investigate the impact of video input channels, fusion methods, and different video representations. We also study the transferability between tasks, and conduct multi-task learning under different settings. The significant gap between our best model and human performance calls for future study for advanced VidL models. VALUE is available at https://value-benchmark.github.io/.

==> supp_table/keywords.tex <==
% \begin{table*}[h]
% \caption{
% Top-20 most frequent nouns and verbs used in subtitles/annotations. Character names have been filtered out from TV/VIOLIN/VLEP.
% }
% \subfloat[Subtitle
% \label{tab:keyword_sub}]{
% \tablestyle{2pt}{1.8} 
% \def\w{175pt} 

% \begin{tabular}{l|L{\w}L{\w}}
% Dataset & Nouns & Verbs\\  
% \shline
% TV & time, something, guy, way, right, man, thing, look, night, anything, god, someone, nothing, life, day, thank, kind, wait, woman, everything &
% know, go, think, want, see, need, tell, say, take, make, let, mean, come, find, give, look, talk, believe, love, feel \\
% \hline
% How2 & bit, way, kind, time, water, today, thing, lot, side, video, music, right, let, something, oil, cup, sugar, top, part, half &
% make, want, go, see, know, use, take, put, need, add, let, show, think, start, give, look, keep, cut, come, say \\
% \hline
% VIOLIN & time, something, god, look, thing, way, right, man, guy, day, night, mom, anything, thank, kind, nothing, wait, life, baby, let & 
% know, go, think, want, see, say, tell, take, need, let, come, make, mean, look, give, love, feel, talk, believe, call \\
% \hline
% VLEP & time, look, kind, something, thing, right, way, man, day, music, lot, everything, let, bit, guy, thank, food, night, place, god &
% know, go, think, see, want, need, make, take, let, say, come, love, look, mean, tell, give, try, feel, find, eat\\
% \hline
% VATEX & way, time, bit, side, look, god, job, alright, thing, kind, hand, man, today, video, day, right, lot, water, thank, something &
% go, know, see, want, make, take, think, let, put, say, come, need, keep, look, use, give, start, show, hold, love\\
% \hline
% YC2 & bit, oil, water, salt, sauce, pepper, time, kind, teaspoon, heat, pan, cup, chicken, onion, half, way, butter, garlic, side, flavor &
% add, want, make, put, use, go, take, let, see, cook, know, need, give, mix, start, cut, keep, turn, think, look\\
% \end{tabular}
% }

% \subfloat[Query/Question/Caption
% \label{tab:keyword_ann}]{
% \tablestyle{2pt}{1.8} 
% \def\w{170pt} 

% \begin{tabular}{l|L{\w}L{\w}}
% Dataset & Nouns & Verbs\\  
% \shline
% TVR/TVC & walk, hand, room, door, table, conversation, patient, man, phone, woman, apartment, head, talk, bed, front, chair, coffee, arm, tell, couch 
% & talking, walk, take, look, put, sitting, stand, turn, open, holding, sits, tell, hold, pick, asks, say, standing, give, go, looking\\
% TVQA & & \\
% How2R & man, woman, video, lady, person, car, bowl, paper, hand, ingredient, girl, food, piece, plant, water, pan, glass, guy, kitchen, chef
% & make, explain, talking, show, using, showing, making, explaining, put, add, explains, cut, shown, cooking, describes, cutting, hold, holding, use, take\\
% How2QA & video, color, man, woman, person, lady, hand, name, kind, type, bowl, food, ingredient, shirt, car, girl, item, table, boy, paper
% & used, shown, talking, using, put, wearing, added, make, holding, use, seen, cut, hold, want, mentioned, making, add, show, happen, explain\\
% VIOLIN & man, woman, shirt, suit, hair, jacket, blonde, girl, lady, brunette, dress, boy, sweater, grey, friend, room, blue, men, pink, guy
% & wearing, tell, want, asks, sitting, say, explains, talking, trying, haired, see, go, think, make, walk, take, know, holding, going, look\\
% VLEP & man, food, door, tell, room, woman, hand, patient, table, phone, shirt, walk, apartment, something, friend, vlogger, baby, girl, question, someone
% & say, tell, take, go, put, asks, look, give, start, walk, make, talk, going, leave, want, open, see, eat, turn, continue\\
% VATEX-EN-R/-C & man, woman, person, people, boy, girl, group, hand, someone, music, child, ball, men, baby, water, room, piece, front, kid, floor & playing, using, sitting, play, holding, talking, standing, showing, make, wearing, shown, dancing, riding, put, show, stand, demonstrating, throw, demonstrates, hold\\
% YC2R/YC2C & pan, oil, onion, salt, water, sauce, pepper, bowl, place, mix, pot, egg, potato, stir, chicken, mixture, slice, powder, butter, heat 
% & add, cut, mix, put, cook, chopped, remove, fry, take, chop, cover, spread, serve, stir, pour, roll, drain, flip, blend, baking\\
% \end{tabular}
% }

% \vspace{-2mm}
% \label{tab:keywords}
% \end{table*}


